User-centered Evaluation of Popularity Bias in Recommender Systems

Recommendation and ranking systems are known to suffer from popularity bias; the tendency of the algorithm to favor a few popular items while under-representing the majority of other items. Prior research has examined various approaches for mitigating popularity bias and enhancing the recommendation of long-tail, less popular, items. The effectiveness of these approaches is often assessed using different metrics to evaluate the extent to which over-concentration on popular items is reduced. However, not much attention has been given to the user-centered evaluation of this bias; how different users with different levels of interest towards popular items are affected by such algorithms. In this paper, we show the limitations of the existing metrics to evaluate popularity bias mitigation when we want to assess these algorithms from the users' perspective and we propose a new metric that can address these limitations. In addition, we present an effective approach that mitigates popularity bias from the user-centered point of view. Finally, we investigate several state-of-the-art approaches proposed in recent years to mitigate popularity bias and evaluate their performances using the existing metrics and also from the users' perspective. Our experimental results using two publicly-available datasets show that existing popularity bias mitigation techniques ignore the users' tolerance towards popular items. Our proposed user-centered method can tackle popularity bias effectively for different users while also improving the existing metrics.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> tables/lastfm_table.tex <==
%\captionsetup[table]{skip=4pt}

\begin{table*}[t]

%\small
\centering
%\setlength{\tabcolsep}{3pt}
\captionof{table}{Results of different algorithms on two datasets. The setting that yields the same precision for all three reranking methods XQ, DM and CP is chosen and the results is reported. Bold values are statistically significant compared to the second best value in each column with significance level of 0.05 ($\alpha$=0.05) } 
\label{tables/lastfm_rankals}
\begin{tabular}{lcccccccl}
\toprule
          &Precision$\uparrow$& Agg-Div$\uparrow$ &$Gini$$\downarrow$ &$UPD$$\downarrow$
          \\\midrule

Base    &0.076& 0.137  &  0.922& 0.466\\
RG    &0.069& 0.145  & 0.915& 0.435\\
XQ &0.073 &0.169  & 0.908&0.424\\
DM & 0.077&0.175  & 0.905 &0.453\\
FS &0.067&0.176 & 0.891 &0.328\\
CP   &0.071& \textbf{0.203}  &  \textbf{0.879}&\textbf{0.246}\\
\bottomrule
\end{tabular}
\end{table*}

==> tables/m_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
% \small
\captionof{table}{Results of different algorithms on two datasets. The setting that yields the same precision for all four re-ranking methods $XQ$, $DM$, $FS$, and $CP$ is chosen and the results are reported. Bold values are statistically significant compared to the second best value in each column with significance level of 0.05 ($\alpha$=0.05). Up arrows indicate larger values are desirable while down arrows indicate smaller values are better. All algorithms are tuned to yield roughly equal precision. }\label{tab:overall}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{lcccccccc}
%\toprule
                                                & \multicolumn{1}{l}{}      & Agg-Div$\uparrow$ & LC$\uparrow$   & Gini$\downarrow$ & IPD$\downarrow$ & UPD$\downarrow$ \\ \bottomrule
\multicolumn{1}{l|}{\multirow{5}{*}{MovieLens}} & \multicolumn{1}{c|}{Base} & 0.029             & 0.003          & 0.950               & 0.534           & 0.610               \\
\multicolumn{1}{l|}{}                           & \multicolumn{1}{c|}{XQ}   & 0.107             & 0.0836         & 0.888                   & 0.333           & 0.485                  \\
\multicolumn{1}{l|}{}                           & \multicolumn{1}{c|}{DM}   & \textbf{0.127}    & \textbf{0.107} & \textbf{0.734}       & 0.343           & 0.478               \\
\multicolumn{1}{l|}{}                           & \multicolumn{1}{c|}{FS}   & 0.07              & 0.054          & 0.904                 & 0.200           & 0.301            \\
\multicolumn{1}{l|}{}                           & \multicolumn{1}{c|}{CP}   & 0.076             & 0.062          & 0.900            & \textbf{0.133}  & \textbf{0.233}  \\ \hline
\multicolumn{1}{l|}{\multirow{5}{*}{Last.fm}}   & \multicolumn{1}{c|}{Base} & 0.131             & 0.089          & 0.942             & 0.470           & 0.594                \\
\multicolumn{1}{l|}{}                           & \multicolumn{1}{c|}{XQ}   & 0.206             & 0.165          & 0.917                & 0.395           & 0.514                  \\
\multicolumn{1}{l|}{}                           & \multicolumn{1}{c|}{DM}   & \textbf{0.393}    & \textbf{0.356} & \textbf{0.749}         & 0.313           & 0.459             \\
\multicolumn{1}{l|}{}                           & \multicolumn{1}{c|}{FS}   & 0.212             & 0.179          & 0.867                 & 0.203           & 0.374                   \\
\multicolumn{1}{l|}{}                           & \multicolumn{1}{c|}{CP}   & 0.260             & 0.233          & 0.831          & \textbf{0.119}  & \textbf{0.281}  \\ \bottomrule
\end{tabular}
\end{table*}

==> tables/movielens_table.tex <==
%\captionsetup[table]{skip=4pt}

\begin{table*}[t]

%\small
\centering
%\setlength{\tabcolsep}{3pt}
\captionof{table}{Results of different algorithms on two datasets. The setting that yields the same precision for all three reranking methods XQ, DM and CP is chosen and the results is reported. Bold values are statistically significant compared to the second best value in each column with significance level of 0.05 ($\alpha$=0.05) } 
\label{tables/movielens_rankals}
\begin{tabular}{lcccccl}
\toprule
           &Precision$\uparrow$& Agg-Div$\uparrow$  &$Gini$$\downarrow$ &$UPD$$\downarrow$
           \\\midrule

Base   &0.327& 0.194   &0.885& 0.368\\
RG    &0.291& 0.20   &0.872& 0.341 \\
XQ &0.309& 0.384   &0.839&0.308\\
DM &0.300& \textbf{0.519} &\textbf{0.623}&0.302\\
FS &0.313&0.198  &0.863&0.268\\
CP   &0.289& 0.281  & 0.831&\textbf{0.152}\\
\bottomrule
\end{tabular}
\end{table*}
